Adaptive Non-Linear Partition of Unity Methods for Scattered Data Interpolation with Discontinuities

Scattered data approximation with discontinuities is challenging due to the Gibbs phenomenon, which significantly reduces accuracy near interfaces. The recently introduced Non-Linear Partition of Unity Method (NL-PUM) addresses this by combining Radial Basis Function (RBF) interpolation with a non-linear Weighted Essentially Non-Oscillatory (WENO) strategy. While effective, NL-PUM's performance relies heavily on two fixed hyperparameters: the RBF shape parameter and the patch radius. This work extends NL-PUM by adapting both hyperparameters locally using Leave-One-Out Cross-Validation (LOOCV) minimized via Global Optimization with Optimistic Improvement (GOOI). Our main innovation is a smoothness indicator linking a discontinuity-aware shrinkage process to LOOCV-based radius selection: patches in smooth regions remain unchanged, while those near discontinuities automatically shrink to avoid crossing the interface. The resulting method, LOOCV-NL-PUM-GOOI, requires no prior knowledge of interface geometry and introduces no extra cost beyond standard adaptive shape parameter selection. Numerical experiments on synthetic test functions with jump discontinuities and a real-data application to Norwegian Fjords elevation data confirm that this approach substantially reduces approximation error near discontinuities while preserving full accuracy in smooth regions.

==> Manuscript/ex_shared.tex <==
% ex_shared.tex
% Shared preamble for the SIAM article and any supplement.
% Place all macros, packages, and shared author/title info here.

% -----------------------------------------------------------------------
% Packages
% -----------------------------------------------------------------------
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{bm}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage[noend]{algpseudocode}
\usepackage{subfigure}

% -----------------------------------------------------------------------
% Math shortcuts
% -----------------------------------------------------------------------
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\PP}{\mathbb{P}}

\DeclareMathOperator{\csch}{csch}

% -----------------------------------------------------------------------
% Author / Title block (used by \maketitle)
% -----------------------------------------------------------------------
\title{Adaptive Non-Linear Partition of Unity Methods for Scattered Data
  Interpolation with Discontinuities%
  \thanks{Submitted to the editors \today.
    \funding{The work of A.H.\ and R.C.\ has been supported by the INdAM Research group
GNCS, the GFI 2025 Project, and the 2024 Project ``Numerical Analysis and
Modelling'' funded by the Department of Mathematics ``Giuseppe Peano'' of
the University of Torino. This research has been accomplished within the
RITA ``Research ITalian network on Approximation,'' the UMI Group TAA
``Approximation Theory and Applications,'' and the SIMAI Activity Group
ANA\&A ``Numerical and Analytical Approximation of Data and Functions with
Applications.'' The work of A.H.\ and D.F.Y.\ has been supported by grant
PID2023-146836NB-I00, funded by MICIU/AEI/10.13039/501100011033 and by
ERDF/EU. The work of D.F.Y.\ and J.R.-A.\ has been supported by GVA project
CIAICO/2024/089.}}}

\author{
  Adeeba Haider%
  \thanks{Department of Mathematics ``Giuseppe Peano,'' University of
    Torino, via Carlo Alberto 10, 10123 Torino, Italy;
    Member of the INdAM Research group GNCS
    (\email{adeeba.haider@unito.it}).}
  \and
  Roberto Cavoretto%
  \thanks{Department of Mathematics ``Giuseppe Peano,'' University of
    Torino, via Carlo Alberto 10, 10123 Torino, Italy;
    Member of the INdAM Research group GNCS
    (\email{roberto.cavoretto@unito.it}).}
  \and
  Juan Ruiz-\'Alvarez%
  \thanks{Departamento de Matem\'{a}tica Aplicada y Estad\'{i}stica,
    Universidad Polit\'{e}cnica de Cartagena, Cartagena, Spain
    (\email{juan.ruiz@universityvalencia.es}).}
  \and
  Dionisio F.\ Y\'{a}\~{n}ez%
  \thanks{Departamento de Matem\'{a}ticas, Universidad de Valencia,
    Valencia, Spain (\email{dionisio.yanez@uv.es}).}
}
